New hard-TeV extreme blazars detected with the MAGIC telescopes

Extreme high-frequency peaked BL Lac objects (EHBLs) are blazars which exhibit extremely energetic synchrotron emission. They also feature non-thermal gamma-ray emission whose peak lies in the very high-energy (VHE, E > 100 GeV) range, and in some sources exceeds 1TeV: this is the case of hard-TeV EHBLs such as 1ES 0229+200. With the aim of increasing the EHBL population, ten targets were observed with the MAGIC telescopes from 2010 to 2017, for a total of 262 h of good quality data. The data were complemented by coordinated Swift observations. The X-ray data analysis confirms that all the sources but two are EHBLs. The sources show only a modest variability and a harder-when-brighter behavior, typical for this class of objects. At VHE gamma rays, three new sources were detected and a hint of signal was found for another new source. In each case the intrinsic spectrum is compatible with the hypothesis of a hard-TeV nature of these EHBLs. The broadband spectral energy distributions (SEDs) of all sources are built and modeled in the framework of a single-zone purely leptonic model. The VHE gamma-ray detected sources were also interpreted with a spine-layer and a proton synchrotron models. The three models provide a good description of the SEDs. However, the resulting parameters differ substantially in the three scenarios, in particular the magnetization parameter. This work presents a first mini-catalog of VHE gamma-ray and multi-wavelength observations of EHBLs.

==> authorlist.tex <==
%\author{Author Name} \affiliation{The worst part of writing a paper on behalf of big collaboration}

% authors 24.06.2019 Format ApJ
%
\collaboration{(MAGIC Collaboration)}


\author[0000-0001-8307-2007]{V.~A.~Acciari} %{1},
\affiliation{Inst. de Astrof\'isica de Canarias, E-38200 La Laguna, and Universidad de La Laguna, Dpto. Astrof\'isica, E-38206 La Laguna, Tenerife, Spain}


\author[0000-0002-5613-7693]{S.~Ansoldi} %{2,23},
\affiliation{Universit\`a di Udine, and INFN Trieste, I-33100 Udine, Italy}
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}


\author[0000-0002-5037-9034]{L.~A.~Antonelli} %{3},
\affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}


\author{A.~Arbet Engels} %{4},
\affiliation{ETH Zurich, CH-8093 Zurich, Switzerland}

\author{K.~Asano} %{23},
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author{D.~Baack} %{5},
\affiliation{Technische Universit\"at Dortmund, D-44221 Dortmund, Germany}

\author[0000-0002-1444-5604]{A.~Babi\'c} %{6},
\affiliation{Croatian Consortium: University of Rijeka, Department of Physics, 51000 Rijeka; University of Split - FESB, 21000 Split; University of Zagreb - FER, 10000 Zagreb; University of Osijek, 31000 Osijek; Rudjer Boskovic Institute, 10000 Zagreb, Croatia}

\author[0000-0002-8008-2485]{B.~Banerjee} %{7},
\affiliation{Saha Institute of Nuclear Physics, HBNI, 1/AF Bidhannagar, Salt Lake, Sector-1, Kolkata 700064, India}

\author[0000-0001-7909-588X]{U.~Barres de Almeida} %{8},
\affiliation{Centro Brasileiro de Pesquisas F\'isicas (CBPF), 22290-180 URCA, Rio de Janeiro (RJ), Brasil}

\author[0000-0002-0965-0259]{J.~A.~Barrio} %{9},
\affiliation{IPARCOS Institute and EMFTEL Department, Universidad Complutense de Madrid, E-28040 Madrid, Spain}

\author[0000-0002-6729-9022]{J.~Becerra Gonz\'alez} %{1},
\affiliation{Inst. de Astrof\'isica de Canarias, E-38200 La Laguna, and Universidad de La Laguna, Dpto. Astrof\'isica, E-38206 La Laguna, Tenerife, Spain}

\author[0000-0003-0605-108X]{W.~Bednarek} %{10},
\affiliation{University of \L\'od\'z, Department of Astrophysics, PL-90236 \L\'od\'z, Poland}

\author{L.~Bellizzi} %{11},
\affiliation{Universit\`a di Siena and INFN Pisa, I-53100 Siena, Italy}

\author[0000-0003-3108-1141]{E.~Bernardini} %{12,16},
\affiliation{Deutsches Elektronen-Synchrotron (DESY), D-15738 Zeuthen, Germany}
\affiliation{Universit\`a di Padova and INFN, I-35131 Padova, Italy}

\author[0000-0003-0396-4190]{A.~Berti} %{13},
\affiliation{Istituto Nazionale Fisica Nucleare (INFN), 00044 Frascati (Roma) Italy}

\author{J.~Besenrieder} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author[0000-0003-4751-0414]{W.~Bhattacharyya} %{12},
\affiliation{Deutsches Elektronen-Synchrotron (DESY), D-15738 Zeuthen, Germany}

\author[0000-0003-3293-8522]{C.~Bigongiari} %{3},
\affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}

\author[0000-0002-1288-833X]{A.~Biland} %{4},
\affiliation{ETH Zurich, CH-8093 Zurich, Switzerland}

\author[0000-0002-8380-1633]{O.~Blanch} %{15},
\affiliation{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}

\author[0000-0003-2464-9077]{G.~Bonnoli} %{11},
\affiliation{Universit\`a di Siena and INFN Pisa, I-53100 Siena, Italy}

\author[0000-0002-6551-4913]{\v{Z}.~Bo\v{s}njak} %{6},
\affiliation{Croatian Consortium: University of Rijeka, Department of Physics, 51000 Rijeka; University of Split - FESB, 21000 Split; University of Zagreb - FER, 10000 Zagreb; University of Osijek, 31000 Osijek; Rudjer Boskovic Institute, 10000 Zagreb, Croatia}

\author[0000-0002-2687-6380]{G.~Busetto} %{16},
\affiliation{Universit\`a di Padova and INFN, I-35131 Padova, Italy}

\author[0000-0002-4137-4370]{R.~Carosi} %{17},
\affiliation{Universit\`a di Pisa, and INFN Pisa, I-56126 Pisa, Italy}

\author{G.~Ceribella} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author[0000-0001-7891-699X]{M. Cerruti}  %{25},
\affiliation{Universitat de Barcelona, ICCUB, IEEC-UB, E-08028 Barcelona, Spain}

\author[0000-0003-2816-2821]{Y.~Chai} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author[0000-0002-2018-9715]{A.~Chilingaryan} %{18},
\affiliation{The Armenian Consortium: ICRANet-Armenia at NAS RA, A. Alikhanyan National Laboratory}

\author{S.~Cikota} %{6},
\affiliation{Croatian Consortium: University of Rijeka, Department of Physics, 51000 Rijeka; University of Split - FESB, 21000 Split; University of Zagreb - FER, 10000 Zagreb; University of Osijek, 31000 Osijek; Rudjer Boskovic Institute, 10000 Zagreb, Croatia}

\author[0000-0001-7793-3106]{S.~M.~Colak} %{15},
\affiliation{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}

\author{U.~Colin} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author[0000-0002-3700-3745]{E.~Colombo} %{1},
\affiliation{Inst. de Astrof\'isica de Canarias, E-38200 La Laguna, and Universidad de La Laguna, Dpto. Astrof\'isica, E-38206 La Laguna, Tenerife, Spain}

\author[0000-0001-7282-2394]{J.~L.~Contreras} %{9},
\affiliation{IPARCOS Institute and EMFTEL Department, Universidad Complutense de Madrid, E-28040 Madrid, Spain}

\author[0000-0003-4576-0452]{J.~Cortina} %{19},
\affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas, E-28040 Madrid, Spain}

\author[0000-0001-9078-5507]{S.~Covino} %{3},
\affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}

\author[0000-0002-7320-5862]{V.~D'Elia} %{3},
\affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}

\author{P.~Da Vela} %{17},
\affiliation{Universit\`a di Pisa, and INFN Pisa, I-56126 Pisa, Italy}

\author[0000-0001-5409-6544]{F.~Dazzi} %{3},
\affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}

\author[0000-0002-3288-2517]{A.~De Angelis} %{16},
\affiliation{Universit\`a di Padova and INFN, I-35131 Padova, Italy}

\author[0000-0003-3624-4480]{B.~De Lotto} %{2},
\affiliation{Universit\`a di Udine, and INFN Trieste, I-33100 Udine, Italy}

\author[0000-0002-9468-4751]{M.~Delfino} %{15,26},
\affiliation{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}
\affiliation{also at Port d'Informaci\'o Cient\'ifica (PIC) E-08193 Bellaterra (Barcelona) Spain}

\author[0000-0002-0166-5464]{J.~Delgado} %{15,26},
\affiliation{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}
\affiliation{also at Port d'Informaci\'o Cient\'ifica (PIC) E-08193 Bellaterra (Barcelona) Spain}

\author[0000-0002-2672-4141]{D.~Depaoli} %{13},
\affiliation{Istituto Nazionale Fisica Nucleare (INFN), 00044 Frascati (Roma) Italy}

\author[0000-0003-4861-432X]{F.~Di Pierro} %{13},
\affiliation{Istituto Nazionale Fisica Nucleare (INFN), 00044 Frascati (Roma) Italy}

\author[0000-0003-0703-824X]{L.~Di Venere} %{13},
\affiliation{Istituto Nazionale Fisica Nucleare (INFN), 00044 Frascati (Roma) Italy}

\author[0000-0001-6974-2676]{E.~Do Souto Espi\~neira} %{15},
\affiliation{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}

\author[0000-0002-9880-5039]{D.~Dominis Prester} %{6},
\affiliation{Croatian Consortium: University of Rijeka, Department of Physics, 51000 Rijeka; University of Split - FESB, 21000 Split; University of Zagreb - FER, 10000 Zagreb; University of Osijek, 31000 Osijek; Rudjer Boskovic Institute, 10000 Zagreb, Croatia}

\author[0000-0002-3066-724X]{A.~Donini} %{2},
\affiliation{Universit\`a di Udine, and INFN Trieste, I-33100 Udine, Italy}

\author{D.~Dorner} %{20},
\affiliation{Universit\"at W\"urzburg, D-97074 W\"urzburg, Germany}

\author[0000-0001-9104-3214]{M.~Doro} %{16},
\affiliation{Universit\`a di Padova and INFN, I-35131 Padova, Italy}

\author[0000-0001-6796-3205]{D.~Elsaesser} %{5},
\affiliation{Technische Universit\"at Dortmund, D-44221 Dortmund, Germany}

\author[0000-0001-8991-7744]{V.~Fallah Ramazani} %{21},
\altaffiliation{Main Author: \href{mailto:vafara@utu.fi}{vafara@utu.fi} (VFR)}
\affiliation{Finnish MAGIC Consortium: Finnish Centre of Astronomy with ESO (FINCA), University of Turku, FI-20014 Turku, Finland; Astronomy Research Unit, University of Oulu, FI-90014 Oulu, Finland}

\author{A.~Fattorini} %{5},
\affiliation{Technische Universit\"at Dortmund, D-44221 Dortmund, Germany}

\author[0000-0002-1137-6252]{G.~Ferrara} %{3},
\affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}

\author[0000-0002-7480-2730]{D.~Fidalgo} %{9},
\affiliation{IPARCOS Institute and EMFTEL Department, Universidad Complutense de Madrid, E-28040 Madrid, Spain}

\author[0000-0002-0709-9707]{L.~Foffano} %{16},
\affiliation{Universit\`a di Padova and INFN, I-35131 Padova, Italy}

\author[0000-0003-2235-0725]{M.~V.~Fonseca} %{9},
\affiliation{IPARCOS Institute and EMFTEL Department, Universidad Complutense de Madrid, E-28040 Madrid, Spain}

\author[0000-0003-2109-5961]{L.~Font} %{22},
\affiliation{Departament de F\'isica, and CERES-IEEC, Universitat Aut\`onoma de Barcelona, E-08193 Bellaterra, Spain}

\author[0000-0001-5880-7518]{C.~Fruck} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author{S.~Fukami} %{23},
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author[0000-0002-8204-6832]{R.~J.~Garc\'ia L\'opez} %{1},
\affiliation{Inst. de Astrof\'isica de Canarias, E-38200 La Laguna, and Universidad de La Laguna, Dpto. Astrof\'isica, E-38206 La Laguna, Tenerife, Spain}

\author[0000-0002-0445-4566]{M.~Garczarczyk} %{12},
\affiliation{Deutsches Elektronen-Synchrotron (DESY), D-15738 Zeuthen, Germany}

\author{S.~Gasparyan} %{18},
\affiliation{The Armenian Consortium: ICRANet-Armenia at NAS RA, A. Alikhanyan National Laboratory}

\author[0000-0001-8442-7877]{M.~Gaug} %{22},
\affiliation{Departament de F\'isica, and CERES-IEEC, Universitat Aut\`onoma de Barcelona, E-08193 Bellaterra, Spain}

\author[0000-0002-9021-2888]{N.~Giglietto} %{13},
\affiliation{Istituto Nazionale Fisica Nucleare (INFN), 00044 Frascati (Roma) Italy}

\author[0000-0002-8651-2394]{F.~Giordano} %{13},
\affiliation{Istituto Nazionale Fisica Nucleare (INFN), 00044 Frascati (Roma) Italy}

\author[0000-0002-4674-9450]{N.~Godinovi\'c} %{6},
\affiliation{Croatian Consortium: University of Rijeka, Department of Physics, 51000 Rijeka; University of Split - FESB, 21000 Split; University of Zagreb - FER, 10000 Zagreb; University of Osijek, 31000 Osijek; Rudjer Boskovic Institute, 10000 Zagreb, Croatia}

\author[0000-0003-0768-2203]{D.~Green} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author[0000-0002-9636-1825]{D.~Guberman} %{15},
\affiliation{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}

\author[0000-0001-8663-6461]{D.~Hadasch} %{23},
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author[0000-0003-0827-5642]{A.~Hahn} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author[0000-0002-3771-4918]{J.~Herrera} %{1},
\affiliation{Inst. de Astrof\'isica de Canarias, E-38200 La Laguna, and Universidad de La Laguna, Dpto. Astrof\'isica, E-38206 La Laguna, Tenerife, Spain}

\author[0000-0001-5591-5927]{J.~Hoang} %{9},
\affiliation{IPARCOS Institute and EMFTEL Department, Universidad Complutense de Madrid, E-28040 Madrid, Spain}

\author[0000-0002-7027-5021]{D.~Hrupec} %{6},
\affiliation{Croatian Consortium: University of Rijeka, Department of Physics, 51000 Rijeka; University of Split - FESB, 21000 Split; University of Zagreb - FER, 10000 Zagreb; University of Osijek, 31000 Osijek; Rudjer Boskovic Institute, 10000 Zagreb, Croatia}

\author[0000-0002-2133-5251]{M.~H\"utten} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author{T.~Inada} %{23},
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author[0000-0003-1096-9424]{S.~Inoue} %{23},
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author{K.~Ishio} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author{Y.~Iwamura} %{23},
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author{L.~Jouvin} %{15},
\affiliation{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}

\author[0000-0002-5289-1509]{D.~Kerszberg} %{15},
\affiliation{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}

\author[0000-0001-9159-9853]{H.~Kubo} %{23},
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author{J.~Kushida} %{23},
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author[0000-0003-2403-913X]{A.~Lamastra} %{3},
\affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}

\author[0000-0002-8269-5760]{D.~Lelas} %{6},
\affiliation{Croatian Consortium: University of Rijeka, Department of Physics, 51000 Rijeka; University of Split - FESB, 21000 Split; University of Zagreb - FER, 10000 Zagreb; University of Osijek, 31000 Osijek; Rudjer Boskovic Institute, 10000 Zagreb, Croatia}

\author[0000-0001-7626-3788]{F.~Leone} %{3},
\affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}

\author[0000-0002-9155-6199]{E.~Lindfors} %{21},
\affiliation{Finnish MAGIC Consortium: Finnish Centre of Astronomy with ESO (FINCA), University of Turku, FI-20014 Turku, Finland; Astronomy Research Unit, University of Oulu, FI-90014 Oulu, Finland}

\author[0000-0002-6336-865X]{S.~Lombardi} %{3},
\affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}

\author[0000-0003-2501-2270]{F.~Longo} %{2,27},
\affiliation{Universit\`a di Udine, and INFN Trieste, I-33100 Udine, Italy}
\affiliation{also at Dipartimento di Fisica, Universit\`a di Trieste, I-34127 Trieste, Italy}

\author[0000-0002-8791-7908]{M.~L\'opez} %{9},
\affiliation{IPARCOS Institute and EMFTEL Department, Universidad Complutense de Madrid, E-28040 Madrid, Spain}

\author[0000-0002-3882-9477]{R.~L\'opez-Coto} %{16},
\affiliation{Universit\`a di Padova and INFN, I-35131 Padova, Italy}

\author[0000-0003-4603-1884]{A.~L\'opez-Oramas} %{1},
\affiliation{Inst. de Astrof\'isica de Canarias, E-38200 La Laguna, and Universidad de La Laguna, Dpto. Astrof\'isica, E-38206 La Laguna, Tenerife, Spain}

\author[0000-0003-4457-5431]{S.~Loporchio} %{13},
\affiliation{Istituto Nazionale Fisica Nucleare (INFN), 00044 Frascati (Roma) Italy}

\author[0000-0002-6395-3410]{B.~Machado de Oliveira Fraga} %{8},
\affiliation{Centro Brasileiro de Pesquisas F\'isicas (CBPF), 22290-180 URCA, Rio de Janeiro (RJ), Brasil}

\author[0000-0003-0670-7771]{C.~Maggio} %{22},
\affiliation{Departament de F\'isica, and CERES-IEEC, Universitat Aut\`onoma de Barcelona, E-08193 Bellaterra, Spain}

\author[0000-0002-5481-5040]{P.~Majumdar} %{7},
\affiliation{Saha Institute of Nuclear Physics, HBNI, 1/AF Bidhannagar, Salt Lake, Sector-1, Kolkata 700064, India}

\author[0000-0002-1622-3116]{M.~Makariev} %{24},
\affiliation{Inst. for Nucl. Research and Nucl. Energy, Bulgarian Academy of Sciences, BG-1784 Sofia, Bulgaria}

\author[0000-0003-4068-0496]{M.~Mallamaci} %{16},
\affiliation{Universit\`a di Padova and INFN, I-35131 Padova, Italy}

\author[0000-0002-5959-4179]{G.~Maneva} %{24},
\affiliation{Inst. for Nucl. Research and Nucl. Energy, Bulgarian Academy of Sciences, BG-1784 Sofia, Bulgaria}

\author[0000-0003-1530-3031]{M.~Manganaro} %{6},
\affiliation{Croatian Consortium: University of Rijeka, Department of Physics, 51000 Rijeka; University of Split - FESB, 21000 Split; University of Zagreb - FER, 10000 Zagreb; University of Osijek, 31000 Osijek; Rudjer Boskovic Institute, 10000 Zagreb, Croatia}

\author{K.~Mannheim} %{20},
\affiliation{Universit\"at W\"urzburg, D-97074 W\"urzburg, Germany}

\author{L.~Maraschi} %{3},
\affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}

\author[0000-0003-3297-4128]{M.~Mariotti} %{16},
\affiliation{Universit\`a di Padova and INFN, I-35131 Padova, Italy}

\author[0000-0002-9763-9155]{M.~Mart\'inez} %{15},
\affiliation{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}

\author[0000-0002-2010-4005]{D.~Mazin} %{14,23},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author[0000-0002-0076-3134]{S.~Mi\'canovi\'c} %{6},
\affiliation{Croatian Consortium: University of Rijeka, Department of Physics, 51000 Rijeka; University of Split - FESB, 21000 Split; University of Zagreb - FER, 10000 Zagreb; University of Osijek, 31000 Osijek; Rudjer Boskovic Institute, 10000 Zagreb, Croatia}

\author[0000-0002-2686-0098]{D.~Miceli} %{2},
\affiliation{Universit\`a di Udine, and INFN Trieste, I-33100 Udine, Italy}

\author{M.~Minev} %{24},
\affiliation{Inst. for Nucl. Research and Nucl. Energy, Bulgarian Academy of Sciences, BG-1784 Sofia, Bulgaria}

\author[0000-0002-1472-9690]{J.~M.~Miranda} %{11},
\affiliation{Universit\`a di Siena and INFN Pisa, I-53100 Siena, Italy}

\author{R.~Mirzoyan} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author[0000-0003-1204-5516]{E.~Molina} %{25},
\affiliation{Universitat de Barcelona, ICCUB, IEEC-UB, E-08028 Barcelona, Spain}

\author[0000-0002-1344-9080]{A.~Moralejo} %{15},
\affiliation{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}

\author[0000-0001-9400-0922]{D.~Morcuende} %{9},
\affiliation{IPARCOS Institute and EMFTEL Department, Universidad Complutense de Madrid, E-28040 Madrid, Spain}

\author[0000-0002-8358-2098]{V.~Moreno} %{22},
\affiliation{Departament de F\'isica, and CERES-IEEC, Universitat Aut\`onoma de Barcelona, E-08193 Bellaterra, Spain}

\author[0000-0001-5477-9097]{E.~Moretti} %{15},
\affiliation{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}

\author[0000-0002-1942-7376]{P.~Munar-Adrover} %{22},
\affiliation{Departament de F\'isica, and CERES-IEEC, Universitat Aut\`onoma de Barcelona, E-08193 Bellaterra, Spain}

\author[0000-0003-4772-595X]{V.~Neustroev} %{21},
\affiliation{Finnish MAGIC Consortium: Finnish Centre of Astronomy with ESO (FINCA), University of Turku, FI-20014 Turku, Finland; Astronomy Research Unit, University of Oulu, FI-90014 Oulu, Finland}

\author[0000-0001-8375-1907]{C.~Nigro} %{12},
\affiliation{Deutsches Elektronen-Synchrotron (DESY), D-15738 Zeuthen, Germany}

\author[0000-0002-1445-8683]{K.~Nilsson} %{21},
\affiliation{Finnish MAGIC Consortium: Finnish Centre of Astronomy with ESO (FINCA), University of Turku, FI-20014 Turku, Finland; Astronomy Research Unit, University of Oulu, FI-90014 Oulu, Finland}

\author[0000-0002-5031-1849]{D.~Ninci} %{15},
\affiliation{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}

\author[0000-0002-1830-4251]{K.~Nishijima} %{23},
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author[0000-0003-1397-6478]{K.~Noda} %{23},
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author[0000-0002-6482-1671]{L.~Nogu\'es} %{15},
\affiliation{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}

\author{S.~Nozaki} %{23},
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author[0000-0002-2239-3373]{S.~Paiano} %{16},
\affiliation{Universit\`a di Padova and INFN, I-35131 Padova, Italy}

\author[0000-0002-4124-5747]{M.~Palatiello} %{2},
\affiliation{Universit\`a di Udine, and INFN Trieste, I-33100 Udine, Italy}

\author[0000-0002-2830-0502]{D.~Paneque} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author[0000-0003-0158-2826]{R.~Paoletti} %{11},
\affiliation{Universit\`a di Siena and INFN Pisa, I-53100 Siena, Italy}

\author[0000-0002-1566-9044]{J.~M.~Paredes} %{25},
\affiliation{Universitat de Barcelona, ICCUB, IEEC-UB, E-08028 Barcelona, Spain}

\author{P.~Pe\~nil} %{9},
\affiliation{IPARCOS Institute and EMFTEL Department, Universidad Complutense de Madrid, E-28040 Madrid, Spain}

\author[0000-0002-7537-7334]{M.~Peresano} %{2},
\affiliation{Universit\`a di Udine, and INFN Trieste, I-33100 Udine, Italy}

\author[0000-0003-1853-4900]{M.~Persic} %{2,28},
\affiliation{Universit\`a di Udine, and INFN Trieste, I-33100 Udine, Italy}
\affiliation{also at INAF-Trieste and Dept. of Physics \& Astronomy, University of Bologna}

\author[0000-0001-9712-9916]{P.~G.~Prada Moroni} %{17},
\affiliation{Universit\`a di Pisa, and INFN Pisa, I-56126 Pisa, Italy}

\author[0000-0003-4502-9053]{E.~Prandini} %{16},
\affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}
\affiliation{Universit\`a di Padova and INFN, I-35131 Padova, Italy}

\author[0000-0001-7387-3812]{I.~Puljak} %{6},
\affiliation{Croatian Consortium: University of Rijeka, Department of Physics, 51000 Rijeka; University of Split - FESB, 21000 Split; University of Zagreb - FER, 10000 Zagreb; University of Osijek, 31000 Osijek; Rudjer Boskovic Institute, 10000 Zagreb, Croatia}

\author[0000-0003-2636-5000]{W.~Rhode} %{5},
\affiliation{Technische Universit\"at Dortmund, D-44221 Dortmund, Germany}

\author[0000-0002-9931-4557]{M.~Rib\'o} %{25},
\affiliation{Universitat de Barcelona, ICCUB, IEEC-UB, E-08028 Barcelona, Spain}

\author[0000-0003-4137-1134]{J.~Rico} %{15},
\affiliation{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}

\author[0000-0002-1218-9555]{C.~Righi} %{3},
\affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}

\author[0000-0001-5471-4701]{A.~Rugliancich} %{17},
\affiliation{Universit\`a di Pisa, and INFN Pisa, I-56126 Pisa, Italy}

\author[0000-0002-3171-5039]{L.~Saha} %{9},
\affiliation{IPARCOS Institute and EMFTEL Department, Universidad Complutense de Madrid, E-28040 Madrid, Spain}

\author[0000-0003-2011-2731]{N.~Sahakyan} %{18},
\affiliation{The Armenian Consortium: ICRANet-Armenia at NAS RA, A. Alikhanyan National Laboratory}

\author{T.~Saito} %{23},
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author{S.~Sakurai} %{23},
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author[0000-0002-7669-266X]{K.~Satalecka} %{12},
\affiliation{Deutsches Elektronen-Synchrotron (DESY), D-15738 Zeuthen, Germany}

\author[0000-0002-9883-4454]{K.~Schmidt} %{5},
\affiliation{Technische Universit\"at Dortmund, D-44221 Dortmund, Germany}

\author{T.~Schweizer} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author[0000-0002-1659-5374]{J.~Sitarek} %{10},
\affiliation{University of \L\'od\'z, Department of Astrophysics, PL-90236 \L\'od\'z, Poland}

\author{I.~\v{S}nidari\'c} %{6},
\affiliation{Croatian Consortium: University of Rijeka, Department of Physics, 51000 Rijeka; University of Split - FESB, 21000 Split; University of Zagreb - FER, 10000 Zagreb; University of Osijek, 31000 Osijek; Rudjer Boskovic Institute, 10000 Zagreb, Croatia}

\author{D.~Sobczynska} %{10},
\affiliation{University of \L\'od\'z, Department of Astrophysics, PL-90236 \L\'od\'z, Poland}

\author[0000-0001-6566-9192]{A.~Somero} %{1},
\affiliation{Inst. de Astrof\'isica de Canarias, E-38200 La Laguna, and Universidad de La Laguna, Dpto. Astrof\'isica, E-38206 La Laguna, Tenerife, Spain}

\author[0000-0002-9430-5264]{A.~Stamerra} %{3},
\affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}

\author[0000-0003-2108-3311]{D.~Strom} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author{M.~Strzys} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author[0000-0002-2692-5891]{Y.~Suda} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author{T.~Suri\'c} %{6},
\affiliation{Croatian Consortium: University of Rijeka, Department of Physics, 51000 Rijeka; University of Split - FESB, 21000 Split; University of Zagreb - FER, 10000 Zagreb; University of Osijek, 31000 Osijek; Rudjer Boskovic Institute, 10000 Zagreb, Croatia}

\author[0000-0002-0574-6018]{M.~Takahashi} %{23},
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author[0000-0003-0256-0995]{F.~Tavecchio} %{3},
\affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}

\author[0000-0002-9559-3384]{P.~Temnikov} %{24},
\affiliation{Inst. for Nucl. Research and Nucl. Energy, Bulgarian Academy of Sciences, BG-1784 Sofia, Bulgaria}

\author[0000-0002-4209-3407]{T.~Terzi\'c} %{6},
\affiliation{Croatian Consortium: University of Rijeka, Department of Physics, 51000 Rijeka; University of Split - FESB, 21000 Split; University of Zagreb - FER, 10000 Zagreb; University of Osijek, 31000 Osijek; Rudjer Boskovic Institute, 10000 Zagreb, Croatia}

\author{M.~Teshima} %{14,23},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}
\affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}

\author[0000-0003-3638-8943]{N.~Torres-Alb\`a} %{25},
\affiliation{Universitat de Barcelona, ICCUB, IEEC-UB, E-08028 Barcelona, Spain}

\author{L.~Tosti} %{13},
\affiliation{Istituto Nazionale Fisica Nucleare (INFN), 00044 Frascati (Roma) Italy}

\author[0000-0002-4495-9331]{V.~Vagelli} %{13},
\affiliation{Istituto Nazionale Fisica Nucleare (INFN), 00044 Frascati (Roma) Italy}

\author[0000-0002-6173-867X]{J.~van Scherpenberg} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author{G.~Vanzo} %{1},
\affiliation{Inst. de Astrof\'isica de Canarias, E-38200 La Laguna, and Universidad de La Laguna, Dpto. Astrof\'isica, E-38206 La Laguna, Tenerife, Spain}

\author[0000-0002-2409-9792]{M.~Vazquez Acosta} %{1},
\affiliation{Inst. de Astrof\'isica de Canarias, E-38200 La Laguna, and Universidad de La Laguna, Dpto. Astrof\'isica, E-38206 La Laguna, Tenerife, Spain}

\author[0000-0002-0069-9195]{C.~F.~Vigorito} %{13},
\affiliation{Istituto Nazionale Fisica Nucleare (INFN), 00044 Frascati (Roma) Italy}

\author[0000-0001-8040-7852]{V.~Vitale} %{13},
\affiliation{Istituto Nazionale Fisica Nucleare (INFN), 00044 Frascati (Roma) Italy}

\author[0000-0003-3444-3830]{I.~Vovk} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author[0000-0002-7504-2083]{M.~Will} %{14},
\affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}

\author[0000-0001-5763-9487]{D.~Zari\'c} %{6},
\affiliation{Croatian Consortium: University of Rijeka, Department of Physics, 51000 Rijeka; University of Split - FESB, 21000 Split; University of Zagreb - FER, 10000 Zagreb; University of Osijek, 31000 Osijek; Rudjer Boskovic Institute, 10000 Zagreb, Croatia}

\nocollaboration

\author[0000-0002-1998-9707]{C.~Arcaro} 
\altaffiliation{Main author:  \href{mailto:cornelia.arcaro@gmail.com}{cornelia.arcaro@gmail.com} (CA)} 
\affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}

\author[0000-0001-8690-6804]{A.~Carosi} 
\affiliation{Laboratoire d’Annecy de Physique des Particules, Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS, LAPP, 74000 Annecy, France}

\author{F.~D'Ammando} 
\affiliation{Istituto di RadioAstronomia, Bologna}

\author{F.~Tombesi} 
\affiliation{Department of Physics, University of Rome “Tor Vergata”, Via della Ricerca Scientifica 1, 00133, Rome, Italy}
\affiliation{Department of Astronomy, University of Maryland, College Park, MD, 20742, USA}
\affiliation{X-ray Astrophysics Laboratory, NASA/Goddard Space Flight Center, Greenbelt, MD, 20771, USA}
\affiliation{INAF - Astronomical Observatory of Rome, via Frascati 33, 00044, Monte Porzio Catone (Rome), Italy}

\author{A.~Lohfink} 
\affiliation{Montana State University, Department of Physics, Montana State University, P.O. Box 173840, Bozeman, MT 59717-3840}

\correspondingauthor{E.~Prandini}
\email{elisaprandini@gmail.com}

%========================================================================
%{1} \affiliation{Inst. de Astrof\'isica de Canarias, E-38200 La Laguna, and Universidad de La Laguna, Dpto. Astrof\'isica, E-38206 La Laguna, Tenerife, Spain}
%{2} \affiliation{Universit\`a di Udine, and INFN Trieste, I-33100 Udine, Italy}
%{3} \affiliation{National Institute for Astrophysics (INAF), I-00136 Rome, Italy}
%{4} \affiliation{ETH Zurich, CH-8093 Zurich, Switzerland}
%{5} \affiliation{Technische Universit\"at Dortmund, D-44221 Dortmund, Germany}
%{6} \affiliation{Croatian Consortium: University of Rijeka, Department of Physics, 51000 Rijeka; University of Split - FESB, 21000 Split; University of Zagreb - FER, 10000 Zagreb; University of Osijek, 31000 Osijek; Rudjer Boskovic Institute, 10000 Zagreb, Croatia}
%{7} \affiliation{Saha Institute of Nuclear Physics, HBNI, 1/AF Bidhannagar, Salt Lake, Sector-1, Kolkata 700064, India}
%{8} \affiliation{Centro Brasileiro de Pesquisas F\'isicas (CBPF), 22290-180 URCA, Rio de Janeiro (RJ), Brasil}
%{9} \affiliation{IPARCOS Institute and EMFTEL Department, Universidad Complutense de Madrid, E-28040 Madrid, Spain}
%{10} \affiliation{University of \L\'od\'z, Department of Astrophysics, PL-90236 \L\'od\'z, Poland}
%{11} \affiliation{Universit\`a di Siena and INFN Pisa, I-53100 Siena, Italy}
%{12} \affiliation{Deutsches Elektronen-Synchrotron (DESY), D-15738 Zeuthen, Germany}
%{13} \affiliation{Istituto Nazionale Fisica Nucleare (INFN), 00044 Frascati (Roma) Italy}
%{14} \affiliation{Max-Planck-Institut f\"ur Physik, D-80805 M\"unchen, Germany}
%{15} \affiliation{Institut de F\'isica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology (BIST), E-08193 Bellaterra (Barcelona), Spain}
%{16} \affiliation{Universit\`a di Padova and INFN, I-35131 Padova, Italy}
%{17} \affiliation{Universit\`a di Pisa, and INFN Pisa, I-56126 Pisa, Italy}
%{18} \affiliation{The Armenian Consortium: ICRANet-Armenia at NAS RA, A. Alikhanyan National Laboratory}
%{19} \affiliation{Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas, E-28040 Madrid, Spain}
%{20} \affiliation{Universit\"at W\"urzburg, D-97074 W\"urzburg, Germany}
%{21} \affiliation{Finnish MAGIC Consortium: Finnish Centre of Astronomy with ESO (FINCA), University of Turku, FI-20014 Turku, Finland; Astronomy Research Unit, University of Oulu, FI-90014 Oulu, Finland}
%{22} \affiliation{Departament de F\'isica, and CERES-IEEC, Universitat Aut\`onoma de Barcelona, E-08193 Bellaterra, Spain}
%{23} \affiliation{Japanese MAGIC Consortium: ICRR, The University of Tokyo, 277-8582 Chiba, Japan; Department of Physics, Kyoto University, 606-8502 Kyoto, Japan; Tokai University, 259-1292 Kanagawa, Japan; RIKEN, 351-0198 Saitama, Japan}
%{24} \affiliation{Inst. for Nucl. Research and Nucl. Energy, Bulgarian Academy of Sciences, BG-1784 Sofia, Bulgaria}
%{25} \affiliation{Universitat de Barcelona, ICCUB, IEEC-UB, E-08028 Barcelona, Spain}
%{26} \affiliation{also at Port d'Informaci\'o Cient\'ifica (PIC) E-08193 Bellaterra (Barcelona) Spain}
%{27} \affiliation{also at Dipartimento di Fisica, Universit\`a di Trieste, I-34127 Trieste, Italy}
%{28} \affiliation{also at INAF-Trieste and Dept. of Physics \& Astronomy, University of Bologna}

